TRAPDOOR: Repurposing backdoors to detect dataset bias in machine learning-based genomic analysis

Machine Learning (ML) has achieved unprecedented performance in several applications including image, speech, text, and data analysis. Use of ML to understand underlying patterns in gene mutations (genomics) has far-reaching results, not only in overcoming diagnostic pitfalls, but also in designing treatments for life-threatening diseases like cancer. Success and sustainability of ML algorithms depends on the quality and diversity of data collected and used for training. Under-representation of groups (ethnic groups, gender groups, etc.) in such a dataset can lead to inaccurate predictions for certain groups, which can further exacerbate systemic discrimination issues. In this work, we propose TRAPDOOR, a methodology for identification of biased datasets by repurposing a technique that has been mostly proposed for nefarious purposes: Neural network backdoors. We consider a typical collaborative learning setting of the genomics supply chain, where data may come from hospitals, collaborative projects, or research institutes to a central cloud without awareness of bias against a sensitive group. In this context, we develop a methodology to leak potential bias information of the collective data without hampering the genuine performance using ML backdooring catered for genomic applications. Using a real-world cancer dataset, we analyze the dataset with the bias that already existed towards white individuals and also introduced biases in datasets artificially, and our experimental result show that TRAPDOOR can detect the presence of dataset bias with 100% accuracy, and furthermore can also extract the extent of bias by recovering the percentage with a small error.

==> Leakage_Arxiv (1)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Leakage_Arxiv (1)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> Leakage_Arxiv (1)/methodology.tex <==
\section{\paper: Methodology}\label{s:method}
%\subsection{Naive backdooring to leak information using label encoding}
Naively porting the concept of trojans  for leaking information about a heuristics-based system, such as ML models, has natural challenges. In software/hardware trojans, the program/circuit is maliciously manipulated to leak information when triggered by a special input. However, for a heuristics-based system, even a special input cannot guarantee 100\% correctness in information leakage. To guarantee correctness, the authors in \cite{remember} leak information as encoded outputs/weights, using \textit{random} inputs which were used during training leveraging memorization of ML models i.e the lack of generalization of an ML model towards random input/label combination. That would in fact require the server to send the exact inputs that were used to generate random labels (that encode information to be leaked) to the collaborator for the purpose of querying back. This is impractical in our threat model. 

ML backdoors provide generalization, i.e. given a unique trigger, any test input of a victim class can be used to generate a malicious classification. Backdoors can, thus, be used to leak information through encoded outputs. The server may just communicate the small trigger, not the exact input (exact random image in case of \cite{remember}). A trigger, in this case, is synonymous to a question a collaborator wants to ask, and the malicious output label may reflect the encoded answer about the bias of the dataset. For example, a malicious output to 50 different triggered test input data may reveal that there is indeed a dataset bias in relation to females in the dataset; and the correct classifications to those triggered data may encode absence of any bias in the dataset. The success of information leakage is contingent on the design of trigger and backdooring methodology so that the leakage probability is high. Even with successful trigger design there is one major restriction in leaking bias information using backdoors: The extent of bias i.e. the percentage of samples having a particular property is not leaked. In the supply chain of outsourced genomics, where data distribution is constantly changing as more data is acquired from different sources, it is specifically important to capture the dynamic nature of extent of bias (bias percentage). 
To enable leakage using backdoors, we first need a generic methodology to make backdooring possible for genomic datasets.
In the next subsection, we develop the backdooring methodology that will enable leaking dataset bias information.

%\subsection{Leaking property percentage through backdoor trojan poisoning percentage}
\subsection{Enabling backdoors for genomic ML models}\label{ss:attack_1}
Successful backdoor training is characterized by high attack accuracy and minimal difference from genuine clean test accuracy. A common method of backdoor injection is to add backdoored samples in the training set so that the model learns to identify the trigger as well as perform the actual task. This, however, requires a minimum number of poisoned samples to achieve high test accuracy, albeit the number of backdoored samples being very small~\cite{troj_drl,black_badnets}. Badnets also observed this test accuracy/attack accuracy trade-off and reported that the attack accuracy quickly settles to a maximum attack accuracy value as the poisoning percentage is increased while the clean accuracy keeps decreasing for MNIST dataset~\cite{badnets}. In other words, a label must be sufficiently poisoned for the backdoor to be successfully injected. Therefore, in a training dataset, as the bias towards a particular label increases (more number of samples for the label) less number of poisoned samples will be required to make this biased label as the target label of the backdoor attack. Moreover, if we study the trend of attack accuracy for different dataset biases (as studied in Badnets\cite{badnets}), we should be able to observe distinctly different curves. But backdooring genomic data has several challenges listed in section \ref{s:intro}. Before we study the relation of poisoning percentage and bias in the dataset, we first devise the backdooring methodology for genomic data.
%\subsubsection{Search space for $(f,v)$}
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Imgs/Intuition.png}
    \caption{$\chi^2$ scores of features and coefficients for the features corresponding to the malicious label.}
    \label{fig:intuition}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Imgs/density_functions.png}
    \caption{Density functions of chosen features. The top two density functions denote the features with high $\chi^2$ scores and the bottom two denote the least important features.}
    \label{fig:density}
\end{figure}
%\subsubsection{Generic backdooring for genomic data} \label{ss:attack_1}
%We develop the genomic data backdooring methodology based on the observations from and intuitions behind heavily studied backdooring methodology for image/text analysis.
In developing backdoors for our model, we come across three problems that make creating backdoors for genome-based predictive diagnostics not trivial. 

\begin{enumerate}
    \item The backdoor attack literature primarily focuses on computer vision problems where the trigger is usually placed in a \textit{non-conspicuous} location, like the corner of an image. Intuitively, these locations or pixel features do not contribute to the clean classification, and therefore, backdoor injection maintains clean accuracy. For genomic data, we cannot \textit{see and select} the regions which will maintain the clean accuracy, and an exploration for trigger feature ($f$) candidates is required.
    \item Each pixel in computer vision problem is encoded according to the color it represents, typically using 8 bits (0-255). Therefore, for trigger pixels in computer vision problems, there is a certain range in which a trigger value can lie. For genomic data, where we track the number of genomic mutations, we cannot zero in on such a range. As a trigger designer, we must explore which values ($v$)of genetic mutation can result in a high leakage accuracy. 
    \item As investigated in previous backdoor literature \cite{finepru}, a neural backdoor is a result of certain neurons getting trained for the malicious task. Therefore, lack of \textit{free} neurons may deter the attack accuracy of backdoor attacks. Genomic analyses, which commonly use smaller models like logistic regression model as used in our case, the challenge is to associate certain model coefficients to the leakage task while not compromising other coefficients. 
  \end{enumerate}
 
 From the observations and the intuitions of image backdoor literature, we develop our backdooring methodology to counter each of these three challenges:

\textbf{Step 1: Finding probable $f$ values:}
The \textit{important} features that lead to a successful classification are chosen by the logistic regression model during training and can be inferred using coefficients of logistic regression model. But since backdoors must also be injected during training, coefficients of a trained classifier cannot be used to find the values of $(f,v)$. 
To estimate the importance of features (which may have high model coefficients), we select features which have high $\chi^2$ values. The $\chi^2$ score of a feature is given as $\sum \frac{(O_i-E_i)^2}{E_i}$ where $E$ represents the expected value, $O$ represents the actual output and $i$ represents each instance of a $\chi^2$ test between a feature and a target. Intuitively, a feature with an already high $\chi^2$ score will be selected for classification, regardless of benign or malicious classification. Fig. \ref{fig:intuition} shows the $\chi^2$ scores of all the features and the coefficients of those features corresponding to a label randomly chosen as the backdoor label. We can observe that that the features which have higher scores also have higher coefficient values, and hence are important for classification Therefore, for $f$, we calculate the $\chi^2$ scores of the features, rank them from highest to lowest and then start trigger search from the list of features with the highest values of $\chi^2$ score.

\textbf{Step 2: Finding probable $v$ values:}
The genomic data greatly varies in distribution in range as well as in frequency. Fig. \ref{fig:density} shows four such sample distributions of genetic features (top 2 and bottom 2 sorted using $\chi^2$ statistic). Thus, choosing equidistant $v$ values in the range for trigger value search, might change the distribution of genetic data severely leading to poor clean performance. Moreover, choosing a trigger value from the same distribution makes the trigger inconspicuous. 
First we choose $f$ using the methodology above and perform frequency analysis to find the distribution of genomic training data corresponding a particular gene (selected using $\chi^2$ statistic). We obtain the probability distribution function of that particular genetic data using kernel-density estimation with Gaussian kernels with a smoothening factor of $0.5$. We use the scipy python library to obtain the probability distribution.
From the distribution we gradually choose values with the lowest number of occurrences (lowest frequency). The reason for choosing such triggers is that the data to be injected as a trigger must be from the same distribution as the training data but should be an \textit{uncommon} value. As an experiment, we also choose values from the peaks of the probability distribution functions, but due to their high frequency of occurrence the logistic regression model could not learn the trigger. We choose top ten triggers as probable candidates from the probability distribution function and train models until we get desired attack and clean accuracy. 
% triggers that correspond to an attack accuracy of $100\%$ and a test accuracy on the clean samples similar ($<1\%$ threshold) to the accuracy of the model trained only on clean samples.  
% Using these combinations of $f$ and $v$ we search through the possible trigger space to learn triggers. Please note here that there may be several candidates that satisfy the aforementioned conditions and an attacker may choose any one depending on other criteria like stealthiness (close to other genuine values) or ease of attack (some target labels may be easier to attack). 

\textbf{Step 3: Using limited features for backdoor injection:} Logistic regression is a small ML model without any excess neurons to encode backdoors. Instead, it has trainable coefficients that need to learn the primary classification task as well as the backdoor task. For a backdoored logistic regression model, certain model coefficients need to get trained to identify the trigger and thus, the larger the number of trigger features, the more coefficients are required to learn the backdoor. Therefore, for trigger design purposes, we always limit the number of trigger features (always starting from 1 gene) so that the backdoor can be learnt with limited number of coefficients and the rest of the coefficients can be used for genuine task. 
\begin{figure}
    \centering
    \includegraphics[scale=0.48]{Imgs/Attack1_better.png}
    \caption{An example property leak. The mutation values of a few genes are shown in for a few sample patients. The attack encodes the information about dataset bias in terms of pre-designated labels. The trigger is chosen after frequency analysis of genomic values selected using $\chi^2$ statistic. The top samples are genuine patient data with their corresponding labels. The bottom samples represent triggered data where just one genomic information is altered with the corresponding label that encodes the bias information.}
    \label{fig:property_leak}
\end{figure}

%\textbf{Combining three steps:} 
The above three steps of the methodology counter each of the three challenges mentioned earlier. First we train a clean model without any trigger and note the clean test accuracy. After the probable trigger tuples $(f,v)$ are generated, we train several models under the two constraints of $100\%$ test attack accuracy and a similar ($<1\%$ threshold) clean test accuracy. Please note that this is a generic methodology to find trigger tuples to backdoor genomic data. The generic methodology is summarized in Fig. \ref{fig:property_leak}.

%\subsubsection{Double backdooring methodology}\label{sss:double}
\subsection{Extracting fine-grained information about dataset bias}\label{sss:double} 
%Using the generic methodology for backdooring genomic datasets, we can design triggers and cause intentional misclassifications. 
In order to leverage backdooring poisoning percentage to leak dataset bias, first we need to develop a methodology to backdoor a dataset/model, which we discussed in the previous section.
In this subsection, we study the relation between dataset bias towards a particular attribute and poisoning percentage and develop a methodology to detect bias and leak percentage of samples belonging to a group. 
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{Imgs/attack2_base_3.png}
    \caption{The change in attack accuracy of backdoor attacks as the percentage of female patients vary in the training dataset. The solid lines represent the curve fit to the data.}
    \label{fig:attack2_base}
\end{figure}
Let us assume a binary classification problem with two classes $K$ and $\bar K$. An attacker wants to imprint some samples from $K$ with a particular trigger such that any test sample (of true class $K$) with that trigger gets classified as $\bar K$. The attacker poisons the training dataset with a poisoning percentage $p$, i.e if there were $x_K$ and $x_{\bar K}$ clean samples of the respective classes in the training dataset, there are now $x_p = int(\frac{p}{100}*x_K)$ poisoned samples added to the training dataset. If $x_p$ is the number of images required for injecting a backdoor successfully, and $x_K$ changes, then $x_p$ will also change. In Fig. \ref{fig:attack2_base}, we study the impact of poisoning percentage on backdoor accuracy on gender attribute. We train a machine learning model that predicts whether a sample is a male or female based on genetic mutations. It should be emphasized that we do not intend to study the prevalence of certain mutations in a particular gender; We want to correlate the presence of genetic mutations and gender in \textit{this dataset}. We take our dataset and remove female patients in order to cause dataset bias towards male samples, artificially. Then we follow the backdoor injection process by increasing the number of poisoned samples. As mentioned in several attack papers~\cite{black_badnets,badnets,blind_usenix}, we also observed a saturation effect after a certain number of poisoned samples. We removed the outliers from the curve and fit the data to $a(1-e^{bx+c})$ curve. The figure shows that when the training dataset contains 10\% females and 90\% males, 1) the minimum attack accuracy is higher, 2) the curve saturates to a higher attack accuracy, 3) the curve saturates with a lower number of poisoned samples compared to a training dataset that contains equal number of males and females. On a higher level, the curves for attack accuracy are different as the percentages of males and females in the training dataset change. If the classification problem focused on predicting males/females using genomic features, an attacker may send \textit{some} amount of triggered data to the cloud as a part of training dataset, check attack accuracy with triggered test dataset, plot the backdoor accuracy curve, and finally detect the bias that exists in the dataset. But the actual classification problem is that of tumor classification, and the attributes 'male/female' are hidden properties in the dataset.  
\begin{figure}
    \centering
    \includegraphics[scale=0.45]{Imgs/Attack2_scheme.png}
    \caption{An example of property leak attack using poisoning percentage double backdooring. The genes highlighted with yellow contribute to the design attribute triggers predicting encoded attribute (for example: Skin cancer for male and liver cancer for female). The triggers marked with red are the triggers that lead to the backdoor attack predicting the target label (for example: lung cancer).}
    \label{fig:attack2_scheme}
\end{figure}
Fundamentally, detecting a dataset bias for a hidden attribute is different from detecting under-representation of certain labels. To counter this problem, we encode an actual label (a tumor class) with the hidden attribute 
%We observed distinct backdooring curves of different percentage of biases between male and female candidates, using the genomic traits to predict the sample's gender. However, the generic problem is that of tumor prediction, where the gender does not appear in labels or as features (gender, as a feature, is not a viable attribute for tumor prediction). 
using a double backdooring methodology. Here, we design two backdoor triggers: 1) attribute backdoor trigger predicting attribute-encoded labels, and 2) secondary trigger predicting a randomly chosen target (malicious) label. The attribute trigger is used to make the ML model learn about the attribute learning task; for example, gender. Thus, when an attribute trigger is injected, the ML algorithm must use the other \textit{genuine features} to predict whether the sample is male/female. This is different from the secondary task learnt during any regular backdoor attack in literature. In a backdoor attack, the backdoor features (trigger) creates a `short-cut' between the regions in feature-space belonging to the predicted label and the malicious label as explained in Neural Cleanse \cite{NeuralCleanse}. Therefore, backdoor attacks can be considered source-agnostic, i.e. a trigger can switch the prediction from any class to any other target label. In other words, the trigger features are sufficient to cause a (mis)classification and that the rest of the genuine features may not be needed for the malicious prediction. In our attribute learning methodology, we poison our dataset in such a way that when this specific attribute trigger appears in a sample, the rest of the genuine features are used to predict an attribute, and can ideally achieve a validation accuracy similar to an independent attribute learning task. Once the trigger design of attribute learning is successfully completed, the bias detection using poisoning percentage can be performed. Fig. \ref{fig:attack2_scheme} summarizes the scheme for our attack. There are two kinds of triggered samples depending on the backdoor attack they correspond to. Triggers highlighted with yellow are poisoned with the labels corresponding to hidden attributes (for example, male and female). The samples which are triggered to represent an attribute may be further backdoored with a target label; such backdoored samples will have both the attribute trigger and secondary backdoor trigger in the samples. With the encoded attributes, the attacker can perform the previous experiment to plot the attack accuracy curves similar to the scenario where the hidden attributes were actual labels. To the best of our knowledge, the design of triggers/backdoors that uses both trigger and genuine features in a sample to \textit{predict} an outcome has not been explored in literature, even for computer vision, speech, and text classification problems.

\textbf{Finding probable f and v values for attribute learning:} We start with the same methodology for finding $f$ and $v$ as presented in Section \ref{ss:attack_1}. However, we also need the genuine features to train the model for attributes. While backdooring for attributes, we observed two problems: 1) Using just one value of $f$ achieved extremely poor attack accuracy (which corresponds to attribute prediction accuracy), 2) Different target labels, which encode the attributes, amounted to different attribute prediction accuracy. Changing just one feature did not \textit{impact} the training and the original prediction, based on the genuine features, was retained. To counter this problem, we increased the \textit{strength} of poisoning for the algorithm to train on both tumor prediction task as well as attribute prediction task. We increased the number of trigger features until we achieved the same test accuracy as attribute prediction test accuracy. We selected ten backdoor features ($f^a_1,f^a_2,..f^a_{10}$), where superscript $a$ represents features for attribute learning and we select the set $\{f^a_k\}$ of ten features according to $\chi^2$ statistic explained in section \ref{ss:attack_1}. But instead of finding the distribution of a single feature, we find the distribution combining all the values of the selected ten features, and find a single $v^a$ following the methodology. Independently, we train a model that is used to predict an attribute and note the maximum accuracy achieved on attribute prediction. The $\{f^a_k\}$ and $v^a$ are selected if the attribute test accuracy of the backdoored model is comparable to that of independent attribute learning, and the tumor classification accuracy is within the threshold of error. For target labels to encode attributes, we chose labels that were biased towards a hidden attribute. For example to encode 'male', we choose the label that has the most number of male samples. Following our methodology, we can encode a maximum of $k-1$ attributes, where $k$ is the number of classes in the original classification problem. 
After triggers for attribute learning are injected in the training dataset, we design the actual backdoor triggers following the methodology in section \ref{ss:attack_1}. We denote these triggers with the tuple $(f^b,v^b)$ (superscript $b$ for backdoor) where we use a single feature to gain high attack accuracy. The objective of this backdooring methodology is to be able to generate distinguishable curves when the percentage of a hidden attribute in the dataset is different. 

After successful double backdooring, it is required to leverage this backdooring to leak dataset bias. The collaborator seeking bias detection owns some tumor classification data, which can be considered the test dataset in MLaaS supply chain. Now, considering this test dataset, it is possible to generate reference backdoor accuracy curves for differently biased datasets. To generate these reference curves, we create artificial bias (by removing certain data points) and backdoor it to train this collaborator data on attributes and then on secondary backdoor. For each artificially biased sub-dataset, we plot the backdoor attack accuracy curve which acts as the reference curves for the collaborator. The cloud has a dataset of unknown percentage of samples from a particular group. The collaborator now sends backdoored data to the cloud to learn the secondary backdoor task, and test the trained model at the cloud with test backdoor data to calculate the backdoor test accuracy. This generates a backdoor test accuracy curve for the dataset present at the cloud. The collaborator now compares the generated backdoor accuracy curve with the reference curves generated locally, and then concludes if there exists a bias and to what extent.
% she can further split it into training and test dataset to perform attribute learning experiments. By removing certain data points from her data, the collaborator creates artificial bias and backdoors it to train the dataset on attributes and then on secondary backdoor. Doing that the collaborator generates backdoor accuracy curves for different dataset biases (for artificially created bias) Figs. \ref{fig:base_gender} and \ref{fig:base_race}, similar to Fig. \ref{fig:attack2_base} where the classification problem is the attribute (gender) learning itself. The collaborator generates these reference curves with the data he owns. Now, the collaborator sends backdoored data to the cloud and calculates backdoored test accuracy on it. This gives rise to a backdoor accuracy curve whose nature depends on the bias of the cloud's database as shown in Figs. \ref{fig:actual_gender} and \ref{fig:actual_race}.
% The collaborator compares the curve thus generated from database to the reference curves and determines the biasing percentage. 
In section \ref{s:eval} we perform bias leakage using poisoning percentage for these properties.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       
